MILES: Making Imitation Learning Easy with Self-Supervision

Data collection in imitation learning often requires significant, laborious human supervision, such as numerous demonstrations, and/or frequent environment resets for methods that incorporate reinforcement learning. In this work, we propose an alternative approach, MILES: a fully autonomous, self-supervised data collection paradigm, and we show that this enables efficient policy learning from just a single demonstration and a single environment reset. MILES autonomously learns a policy for returning to and then following the single demonstration, whilst being self-guided during data collection, eliminating the need for additional human interventions. We evaluated MILES across several real-world tasks, including tasks that require precise contact-rich manipulation such as locking a lock with a key. We found that, under the constraints of a single demonstration and no repeated environment resetting, MILES significantly outperforms state-of-the-art alternatives like imitation learning methods that leverage reinforcement learning. Videos of our experiments and code can be found on our webpage: www.robot-learning.uk/miles.

==> pseudo-algos/check_env_dist.tex <==

\begin{algorithm}[t!]
\caption{CheckEnvDisturbance}\label{algo:disturbance}

\SetAlgoLined
\KwIn{Demonstration observation $o^\zeta_k$, Captured live image $I^k_M$, similarity threshold $\theta$}
\begin{algorithmic}[1]
\STATE Disturbance $\leftarrow$ \textbf{False} \tcp{\footnotesize init environment disturbance variable}
\STATE $I^\zeta_k \in o^\zeta_k$ \tcp{\footnotesize retrieve RGB image $I^\zeta_k$ from the demonstration's observations}
\STATE $[f^1_{I^\zeta_k}, f^2_{I^\zeta_k}, ...]\leftarrow$DINO-ViT($I^\zeta_k$) \tcp{\footnotesize compute DINO-ViT features \cite{amir2021deep, Caron2021EmergingPI} for \textbf{each} image patch $f^x_{I^\zeta_k}$ for the demo waypoint image}
\STATE $[f^1_{I^k_M}, f^2_{I^k_M}, ...]\leftarrow$DINO-ViT($I^k_M$) \tcp{\footnotesize compute DINO-ViT features \cite{amir2021deep, Caron2021EmergingPI} for \textbf{each} image patch $f^x_{I^k_M}$ from the current live environment image (captured after executing the augmentation trajectory).}

\STATE $sim = $AvgCosineSimilarity($[f^1_{I^\zeta_k}, f^2_{I^\zeta_k}, ...], [f^1_{I^k_M}, f^2_{I^k_M}, ...]$)
\IF{$sim < \theta$}
\STATE Disturbance $\leftarrow$ \textbf{True}
\ENDIF


\end{algorithmic}{}
\KwOut{Disturbance}

\end{algorithm}



==> pseudo-algos/check_reachability.tex <==

\begin{algorithm}[t!]
\caption{CheckReachability}\label{algo:reach}

\SetAlgoLined
\KwIn{Demonstration waypoint $w^\zeta_k$}
\begin{algorithmic}[1]
\STATE Reachable $\leftarrow$ \textbf{True} \tcp{\footnotesize init reachability variable}
\STATE $w^k_M\leftarrow$ EE pose \tcp{\footnotesize achieved after executing the augmentation trajectory (comprising $M$ timesteps); read from proprioception}
\STATE Reachable $= (w^k_M == w^\zeta_k)$ \tcp{\footnotesize check whether poses are equal (within the controller's feasible precision)}
\end{algorithmic}{}
\KwOut{Reachable}

\end{algorithm}



==> pseudo-algos/deploy.tex <==

\begin{algorithm}[h!]
\caption{Deploy}\label{algo:deploy}
\SetAlgoLined
\KwIn{Policy $\pi$, Single Demonstration $\zeta$, final data collection timestep $R$}
\begin{algorithmic}[1]
\STATE Capture observation $o$ \tcp{\footnotesize comprising RGB wrist cam image + force-torque feedback}
\STATE Action $a=f_\psi(o)$
\STATE Perform action $a$
\WHILE{$a$ is not the identity transformation}
\STATE Capture observation $o$
\STATE Action $a=f_\psi(o)$
\STATE Perform action $a$
\ENDWHILE
\newline\tcp{\footnotesize if an environment disturbance stopped data collection before the last demo waypoint}

\IF{$R<\text{length}(\zeta)$}
\STATE Replay remaining demo $\{a^\zeta_n\}_{n=R}^N$
\ENDIF

\end{algorithmic}{}


\end{algorithm}



==> pseudo-algos/fuse_augmentations.tex <==

\begin{algorithm}[h!]
\caption{FuseAugmentationsWithDemo}\label{algo:fuse}

\SetAlgoLined
\KwIn{Dataset of augmentation trajectories $\mathcal{D}$, final data collection time step $R$, single demonstration $\zeta$}
\begin{algorithmic}[1]
\STATE $\mathcal{D}_{\textrm{new}}=\{\}$\tcp{\footnotesize init empty dataset to store fused trajectories}
\FOR{$\tau_k$ in $\mathcal{D}$}
\STATE $\zeta_{\text{segment}} = \underbrace{\{(w^\zeta_n, o^\zeta_n, a^\zeta_n)\}_{n=k}^{R}\}}_{\substack{\textrm{demonstration segment from } k_\textrm{th} \\\textrm{demo waypoint to } R_\textrm{th}}}\in\zeta$
\newline
\STATE $\tau_{k_{\textrm{new}}}:=\tau_k \cup \zeta_{\text{segment}}$
\STATE $\mathcal{D}_{\textrm{new}} = \mathcal{D}_{\textrm{new}} \cup \tau_{k_{\textrm{new}}}$
\ENDFOR
\end{algorithmic}{}
\KwOut{$\mathcal{D}_\text{new}$}

\end{algorithm}



==> pseudo-algos/miles_overview_algo.tex <==

\begin{algorithm*}[tbh!]
\SetAlgoLined
\KwIn{Single Task Demonstration: $\zeta = \{(w^\zeta_n, o^\zeta_n, a^\zeta_n)\}_{n=1}^{N}$, Number of augmentation trajectories per demonstration waypoint $Z$, environment disturbance threshold $\theta$ (Default: $\theta=0.94$)}
\begin{algorithmic}[1]
\STATE $\mathcal{D}=\{\}$ \tcp{init empty dataset of augmentation trajectories}
\STATE Reachable $=$ \textbf{True} \tcp{init variable that tracks reachability}
\STATE Disturbance $=$ \textbf{True} \tcp{init variable that tracks environment disturbances}
\STATE $R=0$ \tcp{init variable that stores the timestep when self-supervised data collection stops} 
\STATE Move robot to the initial demonstration pose $w^\zeta_1$
\FOR{\(\mbox{iteration } k=1 \textrm{ to } N\)} 
\STATE $j=1$ \tcp{keeps track of augmentation trajectories per demo waypoint}
\WHILE{$j \leq Z$}
\STATE $\tau_k\leftarrow$\textit{SampleTrajectory}($w^\zeta_k$) (Alg. \ref{algo:sample_traj})
\STATE Reachable $\leftarrow$\textit{CheckReachability}($w^\zeta_k$) (Alg.~\ref{algo:reach})
\IF{Reachable is \textbf{False}}
\STATE \textit{ReturnToDemoWaypoint}($k$, $\zeta$) (Alg.~\ref{algo:return_to_demo_waypoint})
\STATE Break \tcp{exit while loop}
\ENDIF
\STATE $I^k_M\leftarrow$ Capture RGB wrist-cam image \tcp{$M$ is the $M_{th}$ final timestep of $\tau_k$} 
\STATE Disturbance $\leftarrow$ \textit{CheckEnvDisturbance}($o^\zeta_k$, $I^k_M$, $\theta$) (Alg.~\ref{algo:disturbance})
\IF{Disturbance is \textbf{True}}
\STATE $R = k$ \tcp{store timestep when data collection stops}
\STATE Break \tcp{exit while loop}  
\ENDIF
\STATE $\mathcal{D} = \mathcal{D} \cup \tau_k$ \tcp{add augmentation trajectory to dataset}
\STATE $j=j+1$
\ENDWHILE
\IF{Disturbance is \textbf{True}}
\STATE Break \tcp{exit for loop}
\ENDIF
\STATE Proceed to the next demonstration state by performing action $a^\zeta_k$ \tcp{follow the demonstration's progression}
\ENDFOR
\STATE $\mathcal{D}_{\textrm{new}}\leftarrow$\textit{FuseAugmentationsWithDemo}($\mathcal{D}$, $R$, $\zeta$)(Alg.~\ref{algo:fuse})
\STATE $\pi\leftarrow$\textit{TrainPolicy}($\mathcal{D}_{\textrm{new}}$, $R$, $\zeta$)(Alg.~\ref{algo:train_policy})
\STATE \textit{Deploy}($\pi$, $R$, $\zeta$)(Alg.~\ref{algo:deploy})
\caption{\textbf{MILES Overview} (Simplified)}\label{algo:train}
\end{algorithmic}{}
\KwOut{$\pi$}
\end{algorithm*}



==> pseudo-algos/return_to_demo_waypoint.tex <==
\begin{algorithm}[h!]
\caption{ReturnToDemoWaypoint}\label{algo:return_to_demo_waypoint}
\SetAlgoLined
\KwIn{Demonstration timestep $k$, Single Demonstration $\zeta$}
\begin{algorithmic}[1]
\STATE Move to initial demonstration waypoint $w^\zeta_1\in\zeta$
\newline
\tcp{\footnotesize replay demonstration up to the $k_{\textrm{th}}$ timestep}
\FOR{iteration $t=1$ to $t=k$} 
\STATE Perform action $a^\zeta_t\in\zeta$
\ENDFOR
\end{algorithmic}{}
\end{algorithm}

==> pseudo-algos/train_policy.tex <==

\begin{algorithm}[tbh!]
\caption{TrainPolicy}\label{algo:train_policy}
\SetAlgoLined
\KwIn{Dataset of augmentation trajectories + demo $\mathcal{D}_{\text{new}}$, final data collection timestep $R$, single demonstration $\zeta$}
\begin{algorithmic}[1]
\STATE Train neural network $f_\psi$ on $\mathcal{D}_{\text{new}}$ using standard behavioral cloning\tcp{\footnotesize \textbf{Discard} waypoints, only observation inputs are used for $f_\psi$}
\IF{$R<\text{length}(\zeta)$} 
\STATE $\pi = \{f_\psi, \{a^\zeta_n\}_{n=R}^N\}$ \tcp{\footnotesize policy consists of an end-to-end neural net + demo replay (if an environment disturbance stopped data collection before the last demo waypoint)}
\ELSE
\STATE $\pi = \{f_\psi\}$ \tcp{\footnotesize policy consists only of an end-to-end neural net}
\ENDIF
\end{algorithmic}{}
\KwOut{$\pi$}

\end{algorithm}



==> results_table.tex <==
\begin{table}[!thb]

\footnotesize
% \setlength{\tabcolsep}{2pt}
\centering
% \addtolength{\leftskip} {-0.1cm} 
\begin{tabular}{|c|c|c|c|c|c|c|c}
Key-Lock & USB & Power Cable & Plug & Toaster & Lid & Screwdriver \\ \hline
18/20 & 14/20 & 17/20 & 17/20 & 19/20 & 20/20 & 17/20

                                                  
\end{tabular}\caption{Success rate results for 7 different tasks.}\label{tab1}
\vspace{-.55cm}
\end{table}

